Soft Calibration Objectives for Neural Networks

Optimal decision making requires that classifiers produce uncertainty estimates consistent with their empirical accuracy. However, deep neural networks are often under- or over-confident in their predictions. Consequently, methods have been developed to improve the calibration of their predictive uncertainty both during training and post-hoc. In this work, we propose differentiable losses to improve calibration based on a soft (continuous) version of the binning operation underlying popular calibration-error estimators. When incorporated into training, these soft calibration losses achieve state-of-the-art single-model ECE across multiple datasets with less than 1% decrease in accuracy. For instance, we observe an 82% reduction in ECE (70% relative to the post-hoc rescaled ECE) in exchange for a 0.7% relative decrease in accuracy relative to the cross entropy baseline on CIFAR-100. When incorporated post-training, the soft-binning-based calibration error objective improves upon temperature scaling, a popular recalibration method. Overall, experiments across losses and datasets demonstrate that using calibration-sensitive procedures yield better uncertainty estimates under dataset shift than the standard practice of using a cross entropy loss and post-hoc recalibration methods.

==> figures/old_table_backup.tex <==
\begin{table}[h]
\caption{ We report accuracy, ECE, and ECE obtained after post-hoc temperature scaling (TS) for models trained with different objectives on the CIFAR-10, CIFAR-100, and ImageNet datasets. ECE is computed with the $\ell_2$ norm and equal-mass binning. Soft calibration objectives (SB-ECE, S-AvUC) result in better or equivalent ECEs compared to previous methods with or without TS.  We also find that TS does not always improve ECE. The best ECE value is highlighted for each dataset. The best ECE with TS value is highlighted if it improves over the best value from the ECE column.}
%\\ (L2 Equal-Mass ECE)}
\begin{subtable}[c]{0.5\textwidth}
  \subcaption{CIFAR-100}
\label{cifar100-table}
  \centering
  \resizebox{\textwidth}{!}{
  \begin{tabular}{||c||c||c|c||}
    \hline
    Loss Fn. & Accuracy & ECE & \makecell {ECE with  TS} \\
    \hline
    NLL & 78.67 & 9.10 & 5.36 \\
    \hline
    %\makecell {NLL +  MMCE} & 74.91 & 3.87 & 4.56 \\
    \makecell {NLL +  MMCE} & 77.26 & 4.73 & \textbf{4.14} \\
    \hline
    Focal & 78.33 & 4.66 & 6.47 \\
    \hline
    %\makecell {Focal + \\ MMCE} & 78.39 & 7.32 & 4.70 \\
    %\hline
    \makecell {Focal +  SB-ECE} & 78.59 & 2.30 & 5.16 \\
    %\hline
    %Focal + S-AvUC-B & 78.27 & \textbf{1.43} & 4.05 & 2.84 \\
    \hline
    \makecell {Focal +  S-AvUC} & 78.13 & \textbf{1.57} & 4.15 \\
    \hline
  \end{tabular}
  }
\end{subtable} \hfill
\begin{subtable}[c]{0.5\textwidth}
\centering
  \subcaption{CIFAR-10}
\label{cifar10-table}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{||c||c||c|c||}
    \hline
    Loss Fn. & Accuracy & ECE & \makecell {ECE with  TS} \\
    \hline
    NLL & 95.59 & 4.37 & 2.61 \\
    \hline
    \makecell {NLL +  MMCE} & 94.98 & 1.55 & \textbf{1.09} \\
    \hline
    Focal & 94.96 & 5.45 & 2.69 \\
    \hline
    %\makecell {Focal + \\ MMCE} & DNH & DNH & DNH \\
    %\hline
   \makecell {Focal +  SB-ECE} & 95.06 & \textbf{1.19} & 2.08 \\
    %\hline
    %Focal + S-AvUC-B & TBA & TBA & TBA & TBA \\
    \hline
    \makecell {Focal + S-AvUC} & 94.87 & 1.36 & 1.77 \\
    \hline
    %\multicolumn{5}{c}{* DNH denotes that addition of secondary loss did not help}
  \end{tabular}
  }
  %\subcaption{CIFAR-10}
\end{subtable} \\
%\vskip 0.05 in.
\begin{subtable}[c]{0.5\textwidth}
\centering
  \caption{ImageNet}
    \resizebox{\textwidth}{!}{
  \begin{tabular}{||c||c||c|c||}
    \hline
    Loss Fn. & Accuracy & ECE & ECE with TS \\
    \hline
    NLL & 75.84 & 3.83 & 2.20 \\
    \hline
    NLL + MMCE & 75.16 & 3.15 & 2.21 \\
    \hline
    NLL + S-AvUC & 75.59 & \textbf{2.26} & \textbf{2.03} \\
    \hline
    %NLL + S-AvUC-B & 75.41 & 2.89 & \textbf{1.94} & 2.44 \\
    %\hline
    NLL + SB-ECE & 74.71 & 3.12 & 1.94 \\
    \hline
  \end{tabular}}

    \label{imagenet-table}
\end{subtable}
\label{tab:summary_results}
\end{table}
